Robust Neural Abstractive Summarization Systems and Evaluation against Adversarial Information

Sequence-to-sequence (seq2seq) neural models have been actively investigated for abstractive summarization. Nevertheless, existing neural abstractive systems frequently generate factually incorrect summaries and are vulnerable to adversarial information, suggesting a crucial lack of semantic understanding. In this paper, we propose a novel semantic-aware neural abstractive summarization model that learns to generate high quality summaries through semantic interpretation over salient content. A novel evaluation scheme with adversarial samples is introduced to measure how well a model identifies off-topic information, where our model yields significantly better performance than the popular pointer-generator summarizer. Human evaluation also confirms that our system summaries are uniformly more informative and faithful as well as less redundant than the seq2seq model.

==> adversarial.tex <==
%\side{Del}%We argue that high quality summarization models should be robust to noisy content \todo{(like machine translation outputs)} or off-topic information in the input \todo{(like a raw HTML file)}.
%\todo{Even the inclusion of minor irrelevant or unnecessary details in a summary hurts a reader's understanding severely.} 
%However, the recall-based ROUGE and METEOR metrics do not heavily penalize summaries that include irrelevant information.
\comm{what study} Our pilot study suggests that the presence of minor irrelevant details in a summary often hurts a reader's understanding severely, but such an error cannot be captured or penalized by the recall-based ROUGE and METEOR metrics. 

In order to test a model's ability to discern irrelevant information, we design a novel adversarial evaluation scheme, where we purposely mix a limited number of off-topic sentences into a test article. The intuition is that if a summarization system truly understands the salient entities and events, it would ignore unrelated sentences. 
%We randomly select 5,000 articles from the CNN/DM test set with the ``news'' tag in the URL (mainly covering international or domestic events).
% For each article, we randomly insert one to four sentences from articles in the test set with the ``sports'' tag. %in the URL.
% For NYT, we randomly select 5,000 articles from the test set with government related tags (``U.S.'', ``Washington'', ``world'') and insert one to four sentences from articles outside the domain (``arts'', ``sports'', ``technology''). We ensure that sentences containing a pronoun in the first five words are not interrupted from the previous sentence so that discourse chains are unlikely to be broken. %by the operation.
% the content of the article, it would ignore unrelated sentences. We took 15,000 articles from the NYT corpus with government related tags (``u.s.'', ``washington'', ``world''), and for each article, randomly inserted up to four sentences from articles outside the domain (``arts'', ``sports'', ``technology''). We ensured sentences that contained a pronoun in the first five words were not interrupted from the previous sentence so as not to break discourse or coreference chains.

The adversarial evaluation results on seq2seq, pointer-generator, and our shared decoder model are shown in Figure~\ref{fig:adv_eval}, where our model consistently yields significantly better ROUGE-L and METEOR scores than the comparisons, and is less affected as more irrelevant sentences are added. Sample summaries for an adversarial sample are shown in Figure~\ref{fig:adv_ex}. Based on this example and others, we find that our semantic decoder plays an important role in capturing salient predicates and arguments, leading to summaries of better quality. 
